Alkaline CO electro-oxidation: Mechanistic Differences between Copper and Gold Single Crystals and Peculiarities of various Copper Facets

Understanding CO electro-oxidation is crucial towards designing catalysts for electrochemically oxidizing complex organic molecules. Earth-abundant Copper (Cu) has recently been demonstrated to exhibit high alkaline CO electro-oxidation activity, rivaling the previously acclaimed Gold (Au). Herein, we combine single crystal rotating disc electrode (RDE) experiments and ab initio microkinetic modeling to understand the underlying reaction mechanisms on Cu and Au surfaces. Cu exhibits a facet-dependent activity with Cu(111) having a 0.27 V lower overpotential than Au(111) and a comparable CO oxidation current density. Using Koutecky-Levich analysis and DFT based microkinetic modeling, we identify the rate-limiting pathway to be Langmuir-Hinshelwood on Cu whereas Eley-Rideal on Au. We additionally present strikingly variant RDE responses on four Cu facets (111, 100, 110 and 211) and long-term stability analysis on Cu(111) and Au(111). We find a combined reset-reaction profile helps Cu retain its high activity and pose a strong competition to the expensive Au catalysts.

==> cover_letter.tex <==
Potential Reviewers: 
1. Paramaconi Rodriguez (p.b.rodriquez@bham.ac.uk)
2. Maria Escudero/Julia Kunze (julia.kunze@uibk.ac.at)
3. Victor Climent (victor.climent@ua.es)
4. Adam Holewinski (adam.holewinski@colorado.edu)

